Robust Explanatory Analysis for Structured Optimization Networks (REASON) in Learning

We seek a hierarchical resolution of residual error under a composite learning objective as a principled mechanism for identifying and exploiting additional information, particularly under distribution shift and perturbation. Inspired by the System 1/System 2 paradigm, we formulate this principle as a two-loop mechanism serving a common inference goal. A fast, System 1-like loop resolves the residual addressable by the available evidence; the remaining epistemic residual triggers a medium speed, System 2-like loop that actively acquires additional evidence and measures its informational value through residual reduction. Over nested solution spaces, the medium-loop optimum is provably no worse than the fast-loop optimum. Experiments show that the resulting two-loop model consistently improves upon the fast loop at approximately half the computation of the medium loop, including under unseen corruptions, and, when provided a cleaner observation, outperforms staged classifiers and learning-to-defer methods at equal computational cost.

==> tables/w34/T1_main.tex <==
% GENERATED by scripts/w34/build_tables.py; do not edit cells by hand.
% SAME-INPUT protocol throughout: every model reads the degraded observation
% System 1 read.  "One model" is a single medium loop retrained at 392 px,
% 80.31 GMAC by the paper's own pricing, above three of the four cascade costs.
% The delta is cascade minus System 1 with an image-clustered 95 percent
% bootstrap interval (2,000 replicates, a test image resampled with all eight
% of its conditions).  Mean over eight conditions, test split read once.
\begin{table}[t]\centering\setlength{\tabcolsep}{2.0pt}
\caption{One model at the cascade's compute against the cascade, every model
reading the degraded input; mean over eight conditions. S1, S2: System~1,
System~2; the cascade spends $50$ to $54$ percent of S2's compute.}
\label{tab:main}
\begin{tabular}{@{}l rrrr l@{}}
\toprule
 & S1 & One model & S1 $+$ S2 & S2 & $\Delta$ over S1 \\
Benchmark & (\%) & $392$ px & (\%) & $518$ px & (\%) \\
\midrule
Dogs     & 65.17 & 80.07 & 77.94 & 79.53 & $+12.8$ $[12.0{,}13.5]$ \\
CUB      & 57.30 & 72.30 & 69.73 & 72.04 & $+12.4$ $[11.9{,}13.0]$ \\
Aircraft & 69.60 & 74.20 & 77.85 & 73.16 & $+8.3$ $[7.5{,}9.0]$ \\
Pets     & 76.54 & 90.21 & 88.87 & 89.30 & $+12.3$ $[11.7{,}13.0]$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/w34/T2_bracket.tex <==
% GENERATED by scripts/w34/build_tables.py; do not edit cells by hand.
% The three readings of the second observation at one operating point and one
% compute.  re-read: System 2 reads the pixels System 1 read.  independent: an
% INDEPENDENT draw of the same corruption at the same severity.  clean: an
% uncorrupted view, an upper bound on any acquisition.  The first three
% columns are means over all eight conditions.  THE DELTAS ARE READ ON THE
% THREE CONDITIONS WHOSE DEPLOYED DRAW IS A FRESH SAMPLE FROM A CONTINUOUS OR
% NEAR-CONTINUOUS DISTRIBUTION (cutout, noise, blur), where a redraw is a second
% sample from the identical distribution and the comparison is exact; the
% feature mask is matched but its draw is one of five regions, so the gate
% selects unlucky draws and a redraw pays (reported in the prose, W34 round 3);
% on the three graded occlusions the redraw also moves a centered occluder to a
% kinder position and is not claimed.
% Interval: image-clustered bootstrap, 2,000 replicates.
\begin{table}[t]\centering\setlength{\tabcolsep}{2.2pt}
\caption{What a second observation is worth at identical compute: the cascade
when System~2 re-reads, reads an independent draw, or reads a clean view.
Deltas are read on cutout, noise and blur only.}
\label{tab:bracket}
\begin{tabular}{@{}l rrr l r@{}}
\toprule
 & \multicolumn{3}{c}{System 1 $+$ System 2 (\%)} & \multicolumn{2}{c}{$\Delta$ over re-read} \\
\cmidrule(lr){2-4}\cmidrule(l){5-6}
Benchmark & re-read & indep. & clean & independent & clean \\
\midrule
Dogs     & 77.94 & 78.69 & 86.61 & $0.0$ $[-0.3{,}0.4]$ & $+2.7$ \\
CUB      & 69.73 & 72.15 & 87.18 & $-0.1$ $[-0.3{,}0.1]$ & $+2.5$ \\
Aircraft & 77.85 & 77.41 & 91.51 & $0.0$ $[-0.3{,}0.4]$ & $+3.9$ \\
Pets     & 88.87 & 89.34 & 95.06 & $0.0$ $[-0.3{,}0.2]$ & $+1.8$ \\
\bottomrule
\end{tabular}
\end{table}

